The Bit Complexity of Efficient Continuous Optimization

We analyze the bit complexity of efficient algorithms for fundamental optimization problems, such as linear regression, $p$-norm regression, and linear programming (LP). State-of-the-art algorithms are iterative, and in terms of the number of arithmetic operations, they match the current time complexity of multiplying two $n$-by-$n$ matrices (up to polylogarithmic factors). However, previous work has typically assumed infinite precision arithmetic, and due to complicated inverse maintenance techniques, the actual running times of these algorithms are unknown. To settle the running time and bit complexity of these algorithms, we demonstrate that a core common subroutine, known as \emph{inverse maintenance}, is backward-stable. Additionally, we show that iterative approaches for solving constrained weighted regression problems can be accomplished with bounded-error pre-conditioners. Specifically, we prove that linear programs can be solved approximately in matrix multiplication time multiplied by polylog factors that depend on the condition number $\kappa$ of the matrix and the inner and outer radius of the LP problem. $p$-norm regression can be solved approximately in matrix multiplication time multiplied by polylog factors in $\kappa$. Lastly, linear regression can be solved approximately in input-sparsity time multiplied by polylog factors in $\kappa$. Furthermore, we present results for achieving lower than matrix multiplication time for $p$-norm regression by utilizing faster solvers for sparse linear systems.

==> Sec_MWU_2_p.tex <==
\section{Mixed $(2,p)$-Norm Minimization}

\begin{lemma}[\cite{AdilKPS19}]
\label{lemma:all-bounds-w-p}
Let $p\geq 2$, $\ma \in \R^{n\times d}$, $\vb\in\R^d$, and $\vt \in \R^{n}_{\geq 0}$ such that $n^{-1/p}\leq \vt_i \leq 1$, for all $i\in[n]$. Let $\vw \in \R_{\geq 0}^{n}$, and define
$\vwtil_i = (n^{1/p} \vt_i)^{p-2} + \vw_i^{p-2}$ (similar to Step \ref{alg:mwu-p-step-what-2} of Algorithm \ref{alg:mwu-p}). Let
\begin{align*}
\vdeltabar = 
\argmin_{\vdelta: \ma^\top \vdelta = \vb} \gamma_p(\vt,\vdelta), ~~ \text{, and } ~~ \vdeltahat = \argmin_{\vdelta: \ma^\top \vdelta = \vb} \norm{\vdelta}_{\vwtil}^2,
\end{align*}
and suppose $\gamma_p(\vt,\vdeltabar) \leq 1$.
Then
\begin{enumerate}
    \item $\norm{\vdeltabar}_{\vw^{p-2}}^2 \leq \norm{\vw}_p^{p-2}$. \label{lemma:all-bounds-w-p-part-1} 
    
    \item $\norm{\vdeltahat}_{2}^2 \leq \norm{\vdeltahat}_{\vwtil}^2$. \label{lemma:all-bounds-w-p-part-2}
    
    \item $\norm{\vdeltahat}_{\vwtil}^2 \leq n^{(p-2)/p} + \norm{\vw}_p^{p-2}$. \label{lemma:all-bounds-w-p-part-3}
    
    \item $\sum_{i=1}^n \abs{\vdeltahat_i} \abs{\frac{\partial \gamma(n^{1/p}\vt_i, \vw_i)}{\partial \vw_i}} \leq p \cdot  \left(\gamma_p(n^{1/p} \vt, \vw)\right)^{(p-1)/p} + p \cdot n^{(p-2)/(2p)} \cdot \left(\gamma_p(n^{1/p} \vt, \vw)\right)^{1/2}$. \label{lemma:all-bounds-w-p-part-4}
\end{enumerate}
\end{lemma}

\begin{proof}
First note that if $\abs{\vdelta_i}> \vt_i$, then $\gamma_p(\vt_i,\vdelta_i) = \abs{\vdelta_i}^{p} + (\frac{p}{2}-1)\vt_i^p \geq \vt_i^{p-2} \vdelta_i^2$.
Also, if $\abs{\vdelta_i}\leq  \vt_i$, then $\gamma_p(\vt_i,\vdelta_i) = \frac{p}{2} \vt_i^{p-2} \vdelta_i^2 \geq \abs{\vdelta_i}^{p}$. Therefore
\begin{align}
\label{eq:gamma-max-bound}
\gamma_p(\vt_i,\vdelta_i)\geq(\max\{\vt_i,\abs{\vdelta_i}\})^{p-2} \cdot \vdelta_i^2 \geq \abs{\vdelta_i}^p,
\end{align} and since $\gamma_p(\vt,\vdeltabar) \leq 1$,
\begin{align}
\label{eq:deltabar-t-bound}
\norm{\vdeltabar}_p^p \leq 1
~~ \text{, and } ~~ \norm{\vdeltabar}^2_{\vt^{p-2}} \leq 1
\end{align}
By Holder's inequality, we have
\begin{align*}
\norm{\vdeltabar}_{\vw^{p-2}}^2
& = 
\sum_{i=1}^n \vw^{p-2}_i \vdeltabar_i^2
\\ & \leq
\left( \sum_{i=1}^n \left(\vw^{p-2}_i\right)^{p/(p-2)} \right)^{(p-2)/p} \left(\sum_{i=1}^n \left(\vdeltabar_i^2\right)^{p/2}\right)^{2/p}
\\ & = 
\norm{\vw}_p^{p-2} \cdot \norm{\vdeltabar}_p^2,
\end{align*}
and the first part of the lemma follows since $\norm{\vdeltabar}_p^p \leq 1$. The second part follows by noticing that for all $i\in[n]$, $\vwtil_i \geq (n^{1/p} \vt_i)^{p-2} \geq 1$. For the third part, we have
\begin{align*}
\norm{\vdeltahat}_{\vwhat}^2 \leq \norm{\vdeltabar}_{\vwhat}^2 = \sum_{i=1}^n (n^{1/p} \vt_i)^{p-2} \vdeltabar_i^2 + \sum_{i=1}^n \vw_i^{p-2} \vdeltabar_i^2 \leq n^{(p-2)/p} \sum_{i=1}^n \vt_i^{p-2} \vdeltabar_i^2 + \norm{\vw}_p^{p-2} \leq n^{(p-2)/p} + \norm{\vw}_p^{p-2},
\end{align*}
where the penultimate inequality follows from the first part of the lemma, and the last inequality follows from \eqref{eq:deltabar-t-bound}. Now note that
\[
\abs{\frac{\partial \gamma(n^{1/p}\vt_i, \vw_i)}{\partial \vw_i}} = \begin{cases}
p \cdot \left(n^{1/p} \vt_i \right)^{p-2} \vw_i & \text{, if } \abs{\vw_i} \leq n^{1/p} \cdot \vt_i, \\
p \cdot \abs{\vw_i}^{p-2} \vw_i & \text{, otherwise.}
\end{cases}
\]
Therefore
\[
\abs{\frac{\partial \gamma(n^{1/p}\vt_i, \vw_i)}{\partial \vw_i}} = p \cdot \vw_i \cdot \left(\max \{ n^{1/p} \vt_i , \vw_i\} \right)^{p-2}.
\]
Thus by Cauchy-Schwarz inequality, \eqref{eq:gamma-max-bound}, definition of $\vwhat$, and part three of the lemma,
\begin{align*}
\left(\sum_{i=1}^n \abs{\vdeltahat_i} \abs{\frac{\partial \gamma(n^{1/p}\vt_i, \vw_i)}{\partial \vw_i}} \right)^2
& \leq
p^2 \cdot \left(\sum_{i=1}^n \vdeltahat_i^2 \cdot \left(\max \{ n^{1/p} \vt_i , \vw_i\} \right)^{p-2} \right) \cdot \left(\sum_{i=1}^n \vw_i^2 \cdot \left(\max \{ n^{1/p} \vt_i , \vw_i\} \right)^{p-2} \right)
\\ & \leq 
p^2 \cdot \left(\sum_{i=1}^n \vdeltahat_i^2 \cdot \left(\max \{ n^{1/p} \vt_i , \vw_i\} \right)^{p-2} \right) \cdot \gamma_p(n^{1/p} \vt, \vw)
\\ & \leq 
p^2 \cdot \norm{\vdeltahat}_{\vwhat}^2 \cdot \gamma_p(n^{1/p} \vt, \vw)
\\ & \leq
p^2 \cdot \left( n^{(p-2)/p} + \norm{\vw}_p^{p-2} \right) \cdot \gamma_p(n^{1/p} \vt, \vw)
\end{align*}
By \eqref{eq:gamma-max-bound}, we have $\norm{\vw}_p^p \leq \gamma_p(n^{1/p} \vt, \vw)$. Therefore 
\[
\norm{\vw}_p^{p-2} \cdot \gamma_p(n^{1/p} \vt, \vw) \leq \left( \gamma_p(n^{1/p} \vt, \vw) \right)^{1+(p-2)/p} = \left( \gamma_p(n^{1/p} \vt, \vw) \right)^{(2p-2)/p}.
\]
Now since the square root is a concave function, we have
\begin{align*}
\sum_{i=1}^n \abs{\vdeltahat_i} \abs{\frac{\partial \gamma(n^{1/p}\vt_i, \vw_i)}{\partial \vw_i}} 
& \leq 
p \cdot n^{(p-2)/(2p)} \cdot \left(\gamma_p(n^{1/p} \vt, \vw)\right)^{1/2} +
p \cdot  \left(\gamma_p(n^{1/p} \vt, \vw)\right)^{(p-1)/p}.
\end{align*}
\end{proof}



==> Sec_Omitted_Lin_Reg.tex <==
\section{Omitted Proofs of Section \ref{sec:lin_reg}}

\underSample*
\begin{proof}
Let $\ms'=\frac{1}{\sqrt{3\alpha/4}}\ms$. Note that the number of nonzeros of $\ms$ and $\ms'$ are equal. By Lemma \ref{lemma:uniformSampling}, with probability of at least $1-d^{-c/3} - (3/4)^d$, $\frac{1}{\sqrt{1+1/(3\sqrt{\alpha})}} \ms' \ma$ is a $\left( \frac{\sqrt{1+1/(3\sqrt{\alpha})}}{\sqrt{1-1/(3\sqrt{\alpha})}} \right)$-spectral approximation of $\ma$ and $\ms'$ has at most $18\alpha c \norm{\vu}_1 \log d = O(\alpha \norm{\vu}_1 \log d)$ nonzeros. Therefore
with a probability of $1-d^{-c/3} - (3/4)^d$,
\[
\frac{1}{(1+1/(3\sqrt{\alpha}))(3\alpha/4)} \ma^\top \ms^2 \ma=\frac{1}{1+1/(3\sqrt{\alpha})}\ma^\top (\ms')^2 \ma \preceq \ma^\top \ma.
\]
Now note that $(1+1/(3\sqrt{\alpha}))(3\alpha/4)\leq 1$ for $\alpha\in(0,1]$. Therefore $\ma^\top \ms^2 \ma \preceq \ma^\top \ma$. Hence, for all $i\in [n]$, $\tau_i(\ma) \leq \tau_i^{\ms \ma}(\ma)$. Therefore with a probability of $1-d^{-c/3}-(3/4)^d$, for all $i\in [n]$, $\vu'_i$ is a leverage score overestimate. 

Now we bound $\sum_{i=1}^n \vu'_i$. Note that $\textsc{Sample}(\vu, 9\alpha, c)$ and $\textsc{Sample}(\alpha \vu, 9, c)$ are equal in distribution. Therefore by Lemma \ref{lemma:uniformSampling}, $\ms' \ma$ is a $\frac{1}{\sqrt{4/3}}$-spectral approximation of $\ma$ with probability of $1-d^{-c/3}-(3/4)^d$ --- note that this does not add to the probability of failure because one of $1/\sqrt{4/3}$ and $\left( \frac{\sqrt{1+1/(3\sqrt{\alpha})}}{\sqrt{1-1/(3\sqrt{\alpha})}} \right)$ is smaller than the other one and we can use the probability of success of the tighter bound which would imply the other one. Therefore 
\[
\frac{1}{2} \ma^\top \ma \preceq \frac{3}{4} \ma^\top (\ms')^2 \ma = \frac{1}{\alpha} \ma^\top \ms^2 \ma
\]
Hence, for all $i\in [n]$ such that $\va_i \perp \text{ker}(\ms \ma)$,
\[
\tau_i^{\ms \ma}(\ma) \leq \frac{2}{\alpha} \tau_i(\ma),
\]
Now we have
\begin{align*}
\sum_{i=1}^n \vu'_i =\sum_{i=1}^n \min\{\vu_i,\vecv_i\} = \sum_{i=1}^n \vecv_i \leq \sum_{i=1}^n (1+\beta) \tau_i^{\ms \ma}(\ma) \leq \sum_{i=1}^n (1+\beta) \frac{2}{\alpha} \tau_i(\ma) \leq \frac{2d(1+\beta)}{\alpha},
\end{align*}
where the last inequality follows from the fact that the sum of leverage scores is equal to the rank of the matrix.
\end{proof}
